Penalty alternating direction methods for mixed-integer optimal control with combinatorial constraints

We consider mixed-integer optimal control problems with combinatorial constraints that couple over time such as minimum dwell times. We analyze a lifting and decomposition approach into a mixed-integer optimal control problem without combinatorial constraints and a mixed-integer problem for the combinatorial constraints in the control space. Both problems can be solved very efficiently with existing methods such as outer convexification with sum-up-rounding strategies and mixed-integer linear programming techniques. The coupling is handled using a penalty-approach. We provide an exactness result for the penalty which yields a solution approach that convergences to partial minima. We compare the quality of these dedicated points with those of other heuristics amongst an academic example and also for the optimization of electric transmission lines with switching of the network topology for flow reallocation in order to satisfy demands.

==> setup_mp.tex <==
%% Packages
\usepackage[american]{babel}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{lmodern}
% \usepackage{todonotes}
\newcommand{\todo}[1]{}
\usepackage{enumitem}
\usepackage{booktabs}
%\usepackage{notationTRR154}
\usepackage{pgfplots}
\usepackage{relsize}
\usepackage{tikz}
\usepackage{xspace}
\usepackage{csquotes}
\usepackage{hyperref} 
\usepackage{algorithm}
\usepackage{algorithmic} 
\usepackage{cite}

\usepackage{amsmath}
\usepackage{amssymb}

%% Definition of theorem-like environments
%% for most already done in svjour3
\spnewtheorem{assumption}{Assumption}{\bf}{\it}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Moderate Anpassung der Parameter, die TeX bei der
% Berechnung von Zeilenumbrüchen verwendet.
% Siehe: Das LaTeX2e-Sündenregister
\tolerance 1414
\hbadness 1414
\emergencystretch 1.5em
\hfuzz 0.3pt
\widowpenalty=10000
\vfuzz \hfuzz
\raggedbottom

% Abbreviations
\newcommand{\ie}{i.e.,\xspace}  % MP: not space between i. and e. in English
\newcommand{\etc}{etc.\xspace}
\newcommand{\eg}{e.g.,\xspace}  % MP: not space between e. and g. in English
\newcommand{\cf}{see\xspace}
\newcommand{\vs}{vs.\xspace}
\newcommand{\st}{\text{s.t.}\xspace}% MP: not space between s. and t. in English
\newcommand{\fa}{\TRRNotation{\text{for all}\xspace}}%
\newcommand{\etal}{{et\,al.}\xspace}%
\newcommand{\wrt}{{w.r.t.}\xspace}%
\newcommand{\abs}[1]{\mathchoice{\left\lvert #1 \right\rvert}%
{\lvert#1\rvert}%
{\lvert#1\rvert}%
{\lvert#1\rvert}%
}


% Abbreviations
\renewcommand{\:}{\colon}
\newcommand{\Yt}{\ensuremath{Y_t}}
\newcommand{\Ut}{\ensuremath{U_t}}
\newcommand{\Vt}{\ensuremath{V_t}}
\newcommand{\Zt}{\ensuremath{Z_t}}
\newcommand{\Wt}{\ensuremath{V_t}}
\newcommand{\Uc}{\ensuremath{\mathcal{U}}}
\newcommand{\Yc}{\ensuremath{\mathcal{Y}}}
\newcommand{\RR}{\ensuremath{\mathbb{R}}}
\newcommand{\NN}{\ensuremath{\mathbb{N}}}
\newcommand{\rel}{\ensuremath{\mathrm{rel}}}

\DeclareMathOperator{\TV}{TV}
\DeclareMathOperator{\esssup}{ess\,sup}
\DeclareMathOperator{\Vp}{\raisebox{-0.5em}{\ensuremath{+}}\kern-1.0ex\bigvee}
\DeclareMathOperator{\Vm}{\raisebox{-0.5em}{\ensuremath{--}}\kern-1.0ex\bigvee}
\DeclareMathOperator{\Var}{\bigvee}

% math notation
\newcommand{\upto}{\nearrow}
\newcommand{\lOneNorm}[1]{\ensuremath{\mathchoice{\left\lvert #1 \right\rvert}{\lvert#1\rvert}{\lvert#1\rVert}{\lvert#1\rvert}_{l_1}}}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "pde-relax-adm_mp"
%%% End:

